Long-Baseline Neutrino Facility (LBNF) and Deep Underground Neutrino Experiment (DUNE) Conceptual Design Report Volume 2: The Physics Program for DUNE at LBNF

The Physics Program for the Deep Underground Neutrino Experiment (DUNE) at the Fermilab Long-Baseline Neutrino Facility (LBNF) is described.

==> common/acronyms-shared-vol1-4.tex <==
%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\nomenclature{APA}{anode plane assembly} 
\nomenclature{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor}
\nomenclature{CPA}{cathode plane assembly}
\nomenclature{ECAL}{electromagnetic calorimeter}
\nomenclature{GAr}{gaseous argon}
\nomenclature{HV}{high voltage}


==> common/acronyms-vol1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{L1, L2, ...}{WBS level within the LBNF and DUNE Projects, where the overall Project is L1}
\nomenclature{MOU}{memorandum of understanding}
\nomenclature{PIP-II(III)}{Proton Improvement Plan (II or III)}
\nomenclature{SDSTA}{South Dakota Science and Technology Authority}
\nomenclature{WBS}{Work Breakdown Structure}


==> common/acronyms-vol4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
\nomenclature{LNG}{liquefied natural gas}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{PPM/PPB/PPT}{parts per million/billion/trillion}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{SBN}{Short-Baseline Neutrino program (at Fermilab)}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}


==> common/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% COMMON list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{$\mathcal{O}(n)$}{of order $n$}
\nomenclature{3D}{3 dimensional (also 1D, 2D, etc.)} % not phys
\nomenclature{CDR}{Conceptual Design Report}
\nomenclature{CF}{Conventional Facilities}
\nomenclature{CP}{product of charge and parity transformations}
\nomenclature{CPT}{product of charge, parity and time-reversal transformations}
\nomenclature{CPV}{violation of charge and parity symmetry}
\nomenclature{DAQ}{data acquisition}
\nomenclature{DOE}{U.S. Department of Energy}
\nomenclature{DUNE}{Deep Underground Neutrino Experiment}
\nomenclature{ESH}{Environment, Safety and Health}
\nomenclature{eV}{electron-Volt, unit of energy (also keV, MeV, GeV, etc.)}
\nomenclature{FD}{far detector}
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FSCF}{far site conventional facilities}
\nomenclature{NSCF}{near site conventional facilities}
\nomenclature{GUT}{grand unified theory}
\nomenclature{\ktyr}{exposure (without beam), expressed in kilotonnes times years}
\nomenclature{\ktMWyr}{exposure, expressed in kilotonnes $\times$ megawatts $\times$ years} 
\nomenclature{L}{level, indicates depth in feet underground at the far site, e.g., 4850L}
\nomenclature{LAr}{liquid argon}
\nomenclature{LArTPC}{liquid argon time-projection chamber}
\nomenclature{LBL}{long-baseline (physics)}
\nomenclature{LBNF}{Long-Baseline Neutrino Facility}
\nomenclature{MH}{mass hierarchy}
\nomenclature{MI}{Main Injector (at Fermilab)}
\nomenclature{ND}{near neutrino detector}
\nomenclature{NDS}{Near Detector Systems; refers to the collection of detector systems at the near site }
\nomenclature{near detector}{except in Volume 4 Chapter 7, this refers to the \textit{neutrino} detector system in the NDS}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
\nomenclature{POT}{protons on target}
\nomenclature{QA}{quality assurance}
\nomenclature{SM}{Standard Model of particle physics}
\nomenclature{t}{metric ton, written \textit{tonne} (also kt)}
\nomenclature{TPC}{time-projection chamber (not used as `total project cost' in the CDR)}

%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{L1, L2, ...}{WBS level within the LBNF and DUNE Projects, where the overall Project is L1}
\nomenclature{MOU}{memorandum of understanding}
\nomenclature{SDSTA}{South Dakota Science and Technology Authority}
\nomenclature{WBS}{Work Breakdown Structure}


%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{BR}{branching ratio}
\nomenclature{DM}{dark matter}
\nomenclature{DSNB}{Diffuse Supernova Neutrino Background}
\nomenclature{GLoBES}{General Long-Baseline Experiment Simulator (software package)}
\nomenclature{L/E}{length-to-energy ratio}
\nomenclature{LRI}{long-range interactions}
\nomenclature{$M_{\odot}$}{solar mass}
\nomenclature{NC}{neutral current (interaction)}
\nomenclature{NH}{normal (mass) hierarchy}
\nomenclature{NSI}{nonstandard interactions}
\nomenclature{MSW}{Mikheyev-Smirnov-Wolfenstein (effect)}
\nomenclature{SME}{Standard-Model Extension}
\nomenclature{SUSY}{supersymmetry}
\nomenclature{WIMP}{weakly-interacting massive particle}

%%%%%%%%%%%%% PROJECT AND PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{C.L.}{confidence level}

%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\nomenclature{APA}{anode plane assembly} 
\nomenclature{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor}
\nomenclature{CPA}{cathode plane assembly}
\nomenclature{ECAL}{electromagnetic calorimeter}
\nomenclature{GAr}{gaseous argon}
\nomenclature{HV}{high voltage}

%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CC}{charged current (interaction)}
\nomenclature{DIS}{deep inelastic scattering}
\nomenclature{FSI}{final-state interactions}
\nomenclature{GEANT4}{GEometry ANd Tracking, a platform for the simulation of the passage of particles through matter using Monte Carlo methods} 
\nomenclature{GENIE}{Generates Events for Neutrino Interaction Experiments (an object-oriented neutrino Monte Carlo generator)} 
\nomenclature{MC}{Monte Carlo (detector simulation methods)}
\nomenclature{QE}{quasi-elastic (interaction)}

%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{octant}{any of the eight parts into which 4$\pi$ is divided by three mutually perpendicular axes}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}

\fixme{Do we need GVKM, SNO, QCD,  PANDORA,  aTCA and microTCA, AMC, MCH, CPU, GPU, VHDL, OpenCL, PTP, Sync-E, GPS, IEEE, WR}







==> common/init-annex.tex <==
% This should be \input first thing after \begin{document}


\pagestyle{titlepage}

\begin{center}
  {\Huge  \thedoctitle}

  \vspace{10mm}

 {\LARGE \thedocsubtitle}

  \vspace{15mm}

\titleextra

  \vspace{10mm}
  \today
\end{center}

\clearpage

\pagestyle{plain} 

\renewcommand{\familydefault}{\sfdefault}
\renewcommand{\thepage}{\roman{page}}
\setcounter{page}{0}
\cleardoublepage

\setcounter{tocdepth}{3}
\textsf{\tableofcontents}
\clearpage


\textsf{\listoffigures}
\clearpage

\textsf{\listoftables}
\clearpage

%For acronym list to appear just after TOC
%\printnomenclature
\cleardoublepage

\iffinal\else
\textsf{\listoftodos}
\clearpage
\fi

\renewcommand{\thepage}{\arabic{page}}
\setcounter{page}{1}

\pagestyle{fancy}

% Set how header/footers look
\renewcommand{\chaptermark}[1]{%
\markboth{Chapter \thechapter:\ #1}{}}
\fancyhead{}
\fancyhead[RO,LE]{\textsf{\footnotesize \thechapter--\thepage}}
\fancyhead[LO,RE]{\textsf{\footnotesize \leftmark}}

\fancyfoot{}
\fancyfoot[RO]{\textsf{\footnotesize LBNF/DUNE Conceptual Design Report}}
\fancyfoot[LO]{\textsf{\footnotesize \thedoctitle}}
\fancypagestyle{plain}{}

\renewcommand{\headrule}{\vspace{-4mm}\color[gray]{0.5}{\rule{\headwidth}{0.5pt}}}



==> tables/zs-volume-table.tex <==
% do not edit, this is generated by dune-params
% per 40kt DUNE
% name, event rate, event size, data rate, annual data volume
\begin{tabular}[h]{r|r|r|r|r}
\hline
source & event rate & event size & data rate & annual data volume \\
\hline
$^{39}Ar$ & \SI[round-mode=places,round-precision=1]{37.8}{\mega\hertz} & \SI[round-mode=places,round-precision=0]{36.0}{\byte} &
\SI[round-mode=places,round-precision=1]{1.3608}{\giga\byte\per\second} &  \SI[round-mode=places,round-precision=0]{42.9426648664}{\peta\byte}\\
\hline
cosmic-$\mu$ & \SI[round-mode=places,round-precision=3]{0.258947264}{\hertz} &
\SI[round-mode=places,round-precision=1]{50.0}{\kilo\byte} & \SI[round-mode=places,round-precision=1]{12.9473632}{\kilo\byte\per\second} &
\SI[round-mode=places,round-precision=0]{408.57898207}{\giga\byte} \\
\hline
beam-$\nu$ & \SI[round-mode=places,round-precision=0]{10524.2348126}{\per\year} & \SI[round-mode=places,round-precision=1]{10.0}{\mega\byte} &
\SI{3.335}{\kilo\byte\per\second} & \SI[round-mode=places,round-precision=0]{105.242348126}{\giga\byte} \\
\hline
SNB cand. (ZS) & \SI[round-mode=places,round-precision=0]{12.0}{\per\year} & \SI[round-mode=places,round-precision=1]{13.608}{\giga\byte} &
\SI[round-mode=places,round-precision=0]{5174.64851079}{\byte\per\second} & \SI[round-mode=places,round-precision=0]{163.296}{\giga\byte} \\
SNB cand. (FS) & \SI[round-mode=places,round-precision=0]{12.0}{\per\year} & \SI[round-mode=places,round-precision=1]{46.08}{\tera\byte} &
\SI[round-mode=places,round-precision=1]{17.5226192958}{\mega\byte\per\second} & \SI[round-mode=places,round-precision=0]{552.96}{\tera\byte} \\
\hline
\end{tabular}

==> volume-physics/authorlist1.tex <==
% The author list in authblk format
% This file was generated on Dec. 8, 2015, 12:14 p.m. 
% The collaboration listed is as it was on the date: 2015-12-08.
% Retrieved from: dune.bnl.gov/people/members/export/?filename=author-payload-authblk.tex&amp;date=now
% This file was generatd, do not edit this file!
% Contact Maury Goodman for any changes.




\author[43]{R.~Acciarri}
\author[10]{M.~A.~Acero}
\author[43]{M.~Adamowski}
\author[142]{C.~Adams}
\author[43]{P.~Adamson}
\author[133]{Z.~Ahmad}
\author[43]{C.~H.~Albright}
\author[119]{T.~Alion}
\author[129]{E.~Amador}
\author[8]{J.~Anderson}
\author[43]{K.~Anderson}
\author[76]{C.~Andreopoulos}
\author[43]{M.~Andrews}
\author[43]{R.~Andrews}
\author[62]{I.~Anghel}
\author[98]{J.~d.~Anjos}
\author[135]{A.~Ankowski}
\author[72]{M.~Antonello}
\author[31]{A.~Aranda~Fernandez}
\author[13]{A.~Ariga}
\author[13]{T.~Ariga}
\author[75]{D.~Aristizabal}
\author[86]{E.~Arrieta-Diaz}
\author[129]{K.~Aryal}
\author[127]{J.~Asaadi}
\author[102]{D.~Asner}
\author[6]{M.~S.~Athar}
\author[13]{M.~Auger}
\author[29]{A.~Aurisano}
\author[68]{V.~Aushev}
\author[63]{D.~Autiero}
\author[129]{M.~Avila}
\author[137]{J.~J.~Back}
\author[121]{X.~Bai}
\author[105]{B.~Baibussinov}
\author[61]{M.~Baird}
\author[140]{B.~Balantekin}
\author[43]{B.~Baller}
\author[41]{P.~Ballett}
\author[52]{B.~Bambah}
\author[106]{M.~Bansal}
\author[106]{S.~Bansal}
\author[137]{G.~J.~Barker}
\author[83]{W.~A.~Barletta}
\author[101]{G.~Barr}
\author[108]{N.~Barros}
\author[16]{B.~Bartosz}
\author[78]{L.~Bartoszek}
\author[129]{A.~Bashyal}
\author[101]{M.~Bass}
\author[131]{F.~Bay}
\author[99]{J.~Beacom}
\author[106]{B.~R.~Behera}
\author[109]{G.~Bellettini}
\author[26]{V.~Bellini}
\author[16]{O.~Beltramello}
\author[16]{N.~Benekos}
\author[107]{P.~A.~Benetti}
\author[113]{A.~Bercellie}
\author[43]{E.~Berman}
\author[20]{H.~Berns}
\author[43]{R.~Bernstein}
\author[16]{S.~Bertolucci}
\author[49]{B.~Bhandari}
\author[106]{V.~Bhatnagar}
\author[60]{B.~Bhuyan}
\author[89]{J.~Bian}
\author[43]{K.~Biery}
\author[15]{M.~Bishai}
\author[126]{T.~Blackburn}
\author[73]{A.~Blake}
\author[14]{F.~d.~M.~Blaszczyk}
\author[82]{E.~Blaufuss}
\author[123]{B.~Bleakley}
\author[28]{E.~Blucher}
\author[43]{V.~Bocean}
\author[107]{F.~Boffelli}
\author[78]{J.~Boissevain}
\author[116]{S.~Bolognesi}
\author[65]{T.~Bolton}
\author[88]{M.~Bonesini}
\author[33]{T.~Boone}
\author[117]{C.~Booth}
\author[53]{S.~Bordoni}
\author[68]{M.~Borysova}
\author[53]{B.~Bourguille}
\author[137]{S.~B.~Boyd}
\author[73]{D.~Brailsford}
\author[129]{A.~Brandt}
\author[16]{J.~Bremer}
\author[43]{S.~Brice}
\author[86]{C.~Bromberg}
\author[34]{G.~Brooijmans}
\author[129]{G.~Brown}
\author[15]{R.~Brown}
\author[43]{G.~Brunetti}
\author[43]{X.~Bu}
\author[33]{N.~Buchanan}
\author[113]{H.~Budd}
\author[128]{B.~Bugg}
\author[74]{P.~Calafiura}
\author[107]{E.~Calligarich}
\author[17]{E.~Calvo}
\author[34]{L.~Camilleri}
\author[77]{M.~Campanelli}
\author[145]{C.~Cantini}
\author[43]{B.~Carls}
\author[34]{R.~Carr}
\author[77]{M.~Cascella}
\author[44]{C.~Castromonte}
\author[62]{E.~Catano~Mur}
\author[43]{F.~Cavanna}
\author[105]{S.~Centro}
\author[134]{A.~Cervera~Villanueva}
\author[16]{M.~Chalifour}
\author[12]{V.~B.~Chandratre}
\author[129]{A.~Chatterjee}
\author[43]{S.~Chattopadhyay}
\author[133]{S.~Chattopadhyay}
\author[63]{L.~Chaussard}
\author[52]{S.~Chembra}
\author[15]{H.~Chen}
\author[15]{K.~Chen}
\author[21]{M.~Chen}
\author[33]{D.~Cherdack}
\author[34]{C.~Chi}
\author[43]{S.~Childress}
\author[47]{S.~Choubey}
\author[38]{B.~C.~Choudhary}
\author[76]{G.~Christodoulou}
\author[121]{C.~Christofferson}
\author[102]{E.~Church}
\author[81]{D.~Cianci}
\author[124]{T.~Coan}
\author[92]{A.~Cocco}
\author[132]{J.~Coelho}
\author[58]{P.~Cole}
\author[83]{G.~Collin}
\author[83]{J.~M.~Conrad}
\author[114]{M.~Convery}
\author[121]{R.~Corey}
\author[121]{L.~Corwin}
\author[8]{J.~Cranshaw}
\author[145]{P.~Crivelli}
\author[89]{D.~Cronin-Hennessy}
\author[88]{A.~Curioni}
\author[28]{J.~Cushing}
\author[15]{D.~L.~Adams}
\author[58]{D.~Dale}
\author[60]{S.~R.~Das}
\author[115]{T.~Davenne}
\author[61]{G.~S.~Davies}
\author[126]{J.~Davies}
\author[2]{J.~Dawson}
\author[129]{K.~De}
\author[96]{A.~de~Gouvea}
\author[101]{J.~K.~de~Jong}
\author[91]{P.~de~Jong}
\author[8]{P.~De~Lurgio}
\author[91]{M.~Decowski}
\author[116]{A.~Delbart}
\author[115]{C.~Densham}
\author[8]{R.~Dharmapalan}
\author[106]{N.~Dhingra}
\author[145]{S.~Di~Luise}
\author[9]{M.~Diamantopoulou}
\author[61]{J.~S.~Diaz}
\author[113]{G.~Diaz~Bautista}
\author[15]{M.~Diwan}
\author[8]{Z.~Djurcic}
\author[15]{J.~Dolph}
\author[8]{G.~Drake}
\author[71]{D.~Duchesneau}
\author[140]{M.~Duvernois}
\author[119]{H.~Duyang}
\author[74]{D.~A.~Dwyer}
\author[48]{S.~Dye}
\author[110]{S.~Dytman}
\author[114]{B.~Eberly}
\author[50]{R.~Edgecock}
\author[86]{D.~Edmunds}
\author[78]{S.~Elliott}
\author[21]{M.~Elnimr}
\author[116]{S.~Emery}
\author[104]{E.~Endress}
\author[82]{S.~Eno}
\author[13]{A.~Ereditato}
\author[43]{C.~O.~Escobar}
\author[81]{J.~Evans}
\author[107]{A.~Falcone}
\author[126]{L.~Falk}
\author[129]{A.~Farbin}
\author[105]{C.~Farnese}
\author[57]{Y.~Farzan}
\author[105]{A.~Fava}
\author[18]{L.~Favilli}
\author[82]{J.~Felde}
\author[46]{J.~Felix}
\author[4]{S.~Fernandes}
\author[43]{L.~Fields}
\author[73]{A.~Finch}
\author[115]{M.~Fitton}
\author[142]{B.~Fleming}
\author[58]{T.~Forest}
\author[40]{J.~Fowler}
\author[61]{W.~Fox}
\author[15]{J.~Fried}
\author[78]{A.~Friedland}
\author[43]{S.~Fuess}
\author[74]{B.~Fujikawa}
\author[104]{A.~Gago}
\author[132]{H.~Gallagher}
\author[63]{S.~Galymov}
\author[117]{T.~Gamble}
\author[47]{R.~Gandhi}
\author[81]{D.~Garcia-Gamez}
\author[20]{S.~Gardiner}
\author[78]{G.~Garvey}
\author[74]{V.~M.~Gehman}
\author[145]{A.~Gendotti}
\author[15]{G.~d.~Geronimo}
\author[77]{C.~Ghag}
\author[47]{P.~Ghoshal}
\author[105]{D.~Gibin}
\author[17]{I.~Gil-Botella}
\author[15]{R.~Gill}
\author[25]{D.~Girardelli}
\author[55]{A.~Giri}
\author[108]{S.~Glavin}
\author[13]{D.~Goeldi}
\author[65]{S.~Golapinni}
\author[95]{M.~Gold}
\author[44]{R.~A.~Gomes}
\author[134]{J.~J.~Gomez~Cadenas}
\author[8]{M.~C.~Goodman}
\author[56]{D.~Gorbunov}
\author[47]{S.~Goswami}
\author[110]{N.~Graf}
\author[114]{N.~Graf}
\author[114]{M.~Graham}
\author[142]{E.~Gramelini}
\author[90]{R.~Gran}
\author[20]{C.~Grant}
\author[137]{N.~Grant}
\author[26]{V.~Greco}
\author[43]{H.~Greenlee}
\author[140]{L.~Greenler}
\author[79]{C.~Greenley}
\author[29]{M.~Groh}
\author[108]{S.~Grullon}
\author[73]{T.~Grundy}
\author[136]{K.~Grzelak}
\author[78]{E.~Guardincerri}
\author[8]{V.~Guarino}
\author[135]{E.~Guarnaccia}
\author[42]{G.~P.~Guedes}
\author[101]{R.~Guenette}
\author[105]{A.~Guglielmi}
\author[90]{A.~T.~Habig}
\author[15]{R.~W.~Hackenburg}
\author[142]{A.~Hackenburg}
\author[129]{H.~Hadavand}
\author[13]{R.~Haenni}
\author[43]{A.~Hahn}
\author[137]{M.~D.~Haigh}
\author[78]{T.~Haines}
\author[43]{T.~Hamernik}
\author[128]{T.~Handler}
\author[15]{S.~Hans}
\author[43]{D.~Harris}
\author[126]{J.~Hartnell}
\author[67]{T.~Hasegawa}
\author[43]{R.~Hatcher}
\author[128]{A.~Hatzikoutelis}
\author[43]{S.~Hays}
\author[14]{E.~Hazen}
\author[122]{M.~Headley}
\author[43]{A.~Heavey}
\author[142]{K.~Heeger}
\author[122]{J.~Heise}
\author[76]{K.~Hennessy}
\author[81]{J.~Hewes}
\author[49]{A.~Higuera}
\author[58]{T.~Hill}
\author[43]{A.~Himmel}
\author[33]{M.~Hogan}
\author[25]{P.~Holanda}
\author[77]{A.~Holin}
\author[73]{W.~Honey}
\author[145]{S.~Horikawa}
\author[65]{G.~Horton-Smith}
\author[61]{B.~Howard}
\author[43]{J.~Howell}
\author[43]{P.~Hurh}
\author[86]{J.~Huston}
\author[43]{J.~Hylen}
\author[79]{R.~Imlay}
\author[79]{J.~Insler}
\author[107]{G.~Introzzi}
\author[143]{D.~Ioanisyan}
\author[143]{A.~Ioannisian}
\author[113]{K.~Iwamoto}
\author[134]{A.~Izmaylov}
\author[129]{C.~Jackson}
\author[15]{D.~E.~Jaffe}
\author[43]{C.~James}
\author[43]{E.~James}
\author[36]{F.~Jediny}
\author[135]{C.~Jen}
\author[106]{A.~Jhingan}
\author[17]{S.~Jim\'enez}
\author[125]{J.~H.~Jo}
\author[43]{M.~Johnson}
\author[29]{R.~Johnson}
\author[43]{J.~Johnstone}
\author[83]{B.~J.~Jones}
\author[15]{J.~Joshi}
\author[43]{H.~Jostlein}
\author[125]{C.~K.~Jung}
\author[43]{T.~Junk}
\author[59]{A.~Kaboth}
\author[74]{R.~Kadel}
\author[132]{T.~Kafka}
\author[135]{L.~Kalousis}
\author[128]{Y.~Kamyshkov}
\author[81]{G.~Karagiorgi}
\author[9]{D.~Karasavvas}
\author[71]{Y.~Karyotakis}
\author[106]{A.~Kaur}
\author[106]{P.~Kaur}
\author[43]{B.~Kayser}
\author[143]{N.~Kazaryan}
\author[14]{E.~Kearns}
\author[108]{P.~Keener}
\author[129]{S.~Kemboi}
\author[25]{E.~Kemp}
\author[15]{S.~H.~Kettell}
\author[56]{M.~Khabibullin}
\author[58]{M.~Khandaker}
\author[56]{A.~Khotjantsev}
\author[15]{B.~Kirby}
\author[43]{M.~Kirby}
\author[108]{J.~Klein}
\author[43]{T.~Kobilarcik}
\author[19]{S.~Kohn}
\author[43]{G.~Koizumi}
\author[56]{A.~Kopylov}
\author[139]{M.~Kordosky}
\author[73]{L.~Kormos}
\author[16]{U.~Kose}
\author[61]{A.~Kostelecky}
\author[19]{M.~Kramer}
\author[13]{I.~Kreslo}
\author[89]{R.~Kriske}
\author[21]{W.~Kropp}
\author[56]{Y.~Kudenko}
\author[117]{V.~A.~Kudryavtsev}
\author[56]{S.~Kulagin}
\author[106]{A.~Kumar}
\author[69]{G.~Kumar}
\author[48]{J.~Kumar}
\author[106]{L.~Kumar}
\author[79]{T.~Kutter}
\author[4]{A.~Laminack}
\author[108]{K.~Lande}
\author[39]{C.~Lane}
\author[130]{K.~Lang}
\author[15]{F.~Lanni}
\author[48]{J.~Learned}
\author[43]{P.~Lebrun}
\author[78]{D.~Lee}
\author[113]{H.~Lee}
\author[43]{W.~M.~Lee}
\author[1]{M.~A.~Leigui~de~Oliveira}
\author[43]{Q.~Li}
\author[15]{S.~Li}
\author[99]{S.~Li}
\author[125]{X.~Li}
\author[15]{Y.~Li}
\author[40]{Z.~Li}
\author[119]{J.~Libo}
\author[74]{C.~S.~Lin}
\author[33]{S.~Lin}
\author[15]{J.~Ling}
\author[135]{J.~Link}
\author[32]{Z.~Liptak}
\author[15]{D.~Lissauer}
\author[15]{L.~Littenberg}
\author[54]{B.~Littlejohn}
\author[78]{Q.~Liu}
\author[124]{T.~Liu}
\author[43]{S.~Lockwitz}
\author[43]{N.~Lockyer}
\author[74]{T.~Loew}
\author[3]{M.~Lokajicek}
\author[59]{K.~Long}
\author[43]{M.~D.~L.~Lopes}
\author[32]{J.~P.~Lopez}
\author[97]{J.~Losecco}
\author[78]{W.~Louis}
\author[61]{J.~Lowery}
\author[13]{M.~Luethi}
\author[19]{K.~Luk}
\author[43]{B.~Lundberg}
\author[43]{T.~Lundin}
\author[142]{X.~Luo}
\author[53]{T.~Lux}
\author[43]{J.~Lykken}
\author[72]{A.~A.~Machado}
\author[43]{J.~R.~Macier}
\author[8]{S.~Magill}
\author[15]{G.~Mahler}
\author[86]{K.~Mahn}
\author[59]{M.~Malek}
\author[12]{S.~Malhotra}
\author[8]{D.~Malon}
\author[26]{F.~Mammoliti}
\author[8]{S.~Mancina}
\author[38]{S.~K.~Mandal}
\author[52]{S.~Mandodi}
\author[113]{S.~L.~Manly}
\author[132]{A.~Mann}
\author[43]{A.~Marchionni}
\author[15]{W.~Marciano}
\author[135]{C.~Mariani}
\author[48]{J.~Maricic}
\author[32]{A.~Marino}
\author[89]{M.~Marshak}
\author[113]{C.~Marshall}
\author[24]{J.~Marshall}
\author[63]{J.~Marteau}
\author[101]{J.~Martin-Albo}
\author[54]{D.~Martinez}
\author[48]{S.~Matsuno}
\author[79]{J.~Matthews}
\author[78]{C.~Mauger}
\author[76]{K.~Mavrokoridis}
\author[143]{D.~Mayilyan}
\author[116]{E.~Mazzucato}
\author[76]{N.~McCauley}
\author[43]{E.~McCluskey}
\author[117]{N.~McConkey}
\author[111]{K.~McDonald}
\author[113]{K.~S.~McFarland}
\author[113]{A.~M.~McGowan}
\author[125]{C.~McGrew}
\author[139]{R.~McKeown}
\author[58]{D.~McNulty}
\author[123]{R.~McTaggart}
\author[56]{A.~Mefodiev}
\author[33]{M.~Mehrian}
\author[94]{P.~Mehta}
\author[120]{D.~Mei}
\author[134]{O.~Mena}
\author[144]{S.~Menary}
\author[84]{H.~Mendez}
\author[107]{A.~Menegolli}
\author[105]{G.~Meng}
\author[4]{D.~Mertins}
\author[61]{M.~Messier}
\author[79]{W.~Metcalf}
\author[61]{M.~Mewes}
\author[138]{H.~Meyer}
\author[43]{T.~Miao}
\author[48]{R.~Milincic}
\author[89]{W.~Miller}
\author[78]{G.~Mills}
\author[56]{O.~Mineev}
\author[30]{O.~Miranda}
\author[43]{C.~S.~Mishra}
\author[119]{S.~R.~Mishra}
\author[51]{B.~Mitrica}
\author[16]{D.~Mladenov}
\author[103]{I.~Mocioiu}
\author[52]{R.~Mohanta}
\author[43]{N.~Mokhov}
\author[16]{C.~Montanari}
\author[43]{D.~Montanari}
\author[83]{J.~Moon}
\author[15]{M.~Mooney}
\author[43]{C.~Moore}
\author[43]{J.~Morfin}
\author[137]{B.~Morgan}
\author[49]{C.~Morris}
\author[15]{W.~Morse}
\author[83]{Z.~Moss}
\author[43]{C.~Mossey}
\author[1]{C.~A.~Moura}
\author[85]{J.~Mousseau}
\author[23]{L.~Mualem}
\author[138]{M.~Muether}
\author[61]{S.~Mufson}
\author[145]{S.~Murphy}
\author[61]{J.~Musser}
\author[129]{R.~Musser}
\author[74]{Y.~Nakajima}
\author[110]{D.~Naples}
\author[10]{J.~Navarro}
\author[17]{D.~Navas}
\author[139]{J.~Nelson}
\author[16]{M.~Nessi}
\author[108]{M.~Newcomer}
\author[129]{Y.~Ng}
\author[77]{R.~Nichol}
\author[115]{T.~C.~Nicholls}
\author[145]{K.~Nikolics}
\author[61]{E.~Niner}
\author[43]{B.~Norris}
\author[16]{F.~Noto}
\author[15]{P.~Novakova}
\author[134]{P.~Novella}
\author[73]{J.~Nowak}
\author[25]{M.~S.~Nunes}
\author[73]{H.~O'Keeffe}
\author[24]{R.~Oldeman}
\author[25]{R.~Oliveira}
\author[132]{T.~Olson}
\author[68]{Y.~Onishchuk}
\author[43]{J.~Osta}
\author[56]{T.~Ovsjannikova}
\author[86]{B.~Page}
\author[48]{S.~Pakvasa}
\author[117]{S.~Pal}
\author[43]{O.~Palamara}
\author[43]{J.~Paley}
\author[17]{C.~Palomares}
\author[20]{E.~Pantic}
\author[110]{V.~Paolone}
\author[43]{V.~Papadimitriou}
\author[135]{J.~Park}
\author[43]{S.~Parke}
\author[15]{Z.~Parsa}
\author[41]{S.~Pascoli}
\author[23]{R.~Patterson}
\author[74]{S.~Patton}
\author[2]{T.~Patzak}
\author[140]{B.~Paulos}
\author[1]{L.~Paulucci}
\author[43]{Z.~Pavlovic}
\author[89]{G.~Pawloski}
\author[126]{S.~Peeters}
\author[63]{E.~Pennacchio}
\author[77]{A.~Perch}
\author[43]{G.~N.~Perdue}
\author[145]{L.~Periale}
\author[117]{J.~D.~Perkin}
\author[71]{H.~Pessard}
\author[43]{G.~Petrillo}
\author[119]{R.~Petti}
\author[121]{A.~Petukhov}
\author[105]{F.~Pietropaolo}
\author[43]{R.~Plunkett}
\author[43]{S.~Pordes}
\author[15]{M.~Potekhin}
\author[26]{R.~Potenza}
\author[64]{B.~Potukuchi}
\author[120]{N.~Poudyal}
\author[43]{O.~Prokofiev}
\author[106]{N.~Pruthi}
\author[93]{P.~Przewlocki}
\author[43]{D.~Pushka}
\author[15]{X.~Qian}
\author[43]{J.~L.~Raaf}
\author[7]{R.~Raboanary}
\author[15]{V.~Radeka}
\author[139]{A.~Radovic}
\author[43]{I.~Rakhno}
\author[7]{H.~T.~Rakotondramanana}
\author[7]{L.~Rakotondravohitra}
\author[137]{Y.~A.~Ramachers}
\author[43]{R.~Rameika}
\author[78]{J.~Ramsey}
\author[107]{A.~Rappoldi}
\author[107]{G.~Raselli}
\author[73]{P.~Ratoff}
\author[43]{B.~Rebel}
\author[145]{C.~Regenfus}
\author[121]{J.~Reichenbacher}
\author[43]{D.~Reitzner}
\author[71]{A.~Remoto}
\author[49]{A.~Renshaw}
\author[15]{S.~Rescia}
\author[117]{M.~Richardson}
\author[78]{K.~Rielage}
\author[43]{K.~Riesselmann}
\author[117]{M.~Robinson}
\author[114]{L.~Rochester}
\author[25]{O.~B.~Rodrigues}
\author[113]{P.~Rodrigues}
\author[85]{B.~Roe}
\author[48]{M.~Rosen}
\author[43]{R.~M.~Roser}
\author[41]{M.~Ross-Lonergan}
\author[107]{M.~Rossella}
\author[145]{A.~Rubbia}
\author[45]{C.~Rubbia}
\author[43]{R.~Rucinski}
\author[13]{C.~Rudolph~von~Rohr}
\author[142]{B.~Russell}
\author[113]{D.~Ruterbories}
\author[77]{R.~Saakyan}
\author[55]{N.~Sahu}
\author[87]{P.~Sala}
\author[15]{N.~Samios}
\author[53]{F.~Sanchez}
\author[62]{M.~Sanchez}
\author[111]{B.~Sands}
\author[84]{S.~Santana}
\author[17]{R.~Santorelli}
\author[125]{G.~Santucci}
\author[9]{N.~Saoulidou}
\author[87]{A.~Scaramelli}
\author[100]{H.~Schellman}
\author[43]{P.~Schlabach}
\author[43]{R.~Schmitt}
\author[28]{D.~Schmitz}
\author[132]{J.~Schneps}
\author[40]{K.~Scholberg}
\author[43]{A.~Schukraft}
\author[33]{J.~Schwehr}
\author[72]{E.~Segreto}
\author[108]{S.~Seibert}
\author[62]{J.~A.~Sepulveda-Quiroz}
\author[145]{F.~Sergiampietri}
\author[43]{L.~Sexton-Kennedy}
\author[145]{D.~Sgalaberna}
\author[34]{M.~Shaevitz}
\author[106]{J.~Shahi}
\author[129]{S.~Shahsavarani}
\author[43]{P.~Shanahan}
\author[47]{S.~U.~Shankar}
\author[15]{R.~Sharma}
\author[112]{R.~K.~Sharma}
\author[43]{T.~Shaw}
\author[125]{R.~Shrock}
\author[68]{I.~Shyrma}
\author[15]{N.~Simos}
\author[40]{G.~Sinev}
\author[106]{I.~Singh}
\author[106]{J.~Singh}
\author[80]{J.~Singh}
\author[11]{V.~Singh}
\author[78]{G.~Sinnis}
\author[34]{W.~Sippach}
\author[16]{D.~Smargianaki}
\author[21]{M.~Smy}
\author[43]{E.~Snider}
\author[54]{P.~Snopok}
\author[141]{J.~Sobczyk}
\author[21]{H.~Sobel}
\author[127]{M.~Soderberg}
\author[138]{N.~Solomey}
\author[78]{W.~Sondheim}
\author[134]{M.~Sorel}
\author[29]{A.~Sousa}
\author[27]{K.~Soustruznik}
\author[83]{J.~Spitz}
\author[85]{J.~Spitz}
\author[117]{N.~J.~Spooner}
\author[43]{M.~Stancari}
\author[4]{I.~Stancu}
\author[16]{D.~Stefan}
\author[74]{H.~M.~Steiner}
\author[15]{J.~Stewart}
\author[121]{J.~Stock}
\author[51]{S.~Stoica}
\author[14]{J.~Stone}
\author[43]{J.~Strait}
\author[28]{M.~Strait}
\author[43]{T.~Strauss}
\author[43]{S.~Striganov}
\author[93]{R.~Sulej}
\author[82]{G.~Sullivan}
\author[48]{Y.~Sun}
\author[8]{L.~Suter}
\author[26]{C.~M.~Sutera}
\author[20]{R.~Svoboda}
\author[37]{B.~Szczerbinska}
\author[81]{A.~Szelc}
\author[81]{S.~S\"oldner-Rembold}
\author[8]{R.~Talaga}
\author[126]{M.~Tamsett}
\author[43]{S.~Tariq}
\author[58]{E.~Tatar}
\author[61]{R.~Tayloe}
\author[78]{C.~Taylor}
\author[122]{D.~Taylor}
\author[34]{K.~Terao}
\author[117]{M.~Thiesse}
\author[77]{J.~Thomas}
\author[117]{L.~F.~Thompson}
\author[24]{M.~Thomson}
\author[15]{C.~Thorn}
\author[115]{M.~Thorpe}
\author[119]{X.~Tian}
\author[121]{D.~Tiedt}
\author[43]{S.~C.~Timm}
\author[2]{A.~Tonazzo}
\author[43]{T.~Tope}
\author[12]{A.~Topkar}
\author[25]{F.~R.~Torres}
\author[107]{M.~Torti}
\author[134]{M.~Tortola}
\author[26]{F.~Tortorici}
\author[83]{M.~Toups}
\author[76]{C.~Touramanis}
\author[20]{M.~Tripathi}
\author[43]{I.~Tropin}
\author[114]{Y.~Tsai}
\author[74]{K.~V.~Tsang}
\author[118]{R.~Tsenov}
\author[142]{S.~Tufanli}
\author[74]{C.~Tull}
\author[41]{J.~Turner}
\author[79]{M.~Tzanov}
\author[9]{E.~Tziaferi}
\author[59]{Y.~Uchida}
\author[61]{J.~Urheim}
\author[114]{T.~Usher}
\author[66]{M.~Vagins}
\author[139]{P.~Vahle}
\author[5]{G.~A.~Valdiviesso}
\author[43]{L.~Valerio}
\author[125]{Z.~Vallari}
\author[134]{J.~Valle}
\author[108]{R.~Van~Berg}
\author[78]{R.~Van~de~Water}
\author[8]{P.~Van~Gemmeren}
\author[105]{F.~Varanini}
\author[48]{G.~Varner}
\author[116]{G.~Vasseur}
\author[43]{K.~Vaziri}
\author[43]{G.~Velev}
\author[105]{S.~Ventura}
\author[17]{A.~Verdugo}
\author[145]{T.~Viant}
\author[25]{T.~V.~Vieira}
\author[72]{C.~Vignoli}
\author[125]{C.~Vilela}
\author[15]{B.~Viren}
\author[36]{T.~Vrba}
\author[70]{T.~Wachala}
\author[140]{D.~Wahl}
\author[117]{M.~Wallbank}
\author[20]{N.~Walsh}
\author[124]{B.~Wang}
\author[22]{H.~Wang}
\author[120]{L.~Wang}
\author[41]{T.~Wang}
\author[117]{T.K.~Warburton}
\author[33]{D.~Warner}
\author[59]{M.~Wascko}
\author[77]{D.~Waters}
\author[129]{T.~B.~Watson}
\author[115]{A.~Weber}
\author[13]{M.~Weber}
\author[120]{W.~Wei}
\author[62]{A.~Weinstein}
\author[121]{D.~Wells}
\author[140]{D.~Wenman}
\author[62]{M.~Wetstein}
\author[129]{A.~White}
\author[49]{L.~Whitehead}
\author[61]{D.~Whittington}
\author[125]{M.~Wilking}
\author[43]{J.~Willhite}
\author[43]{P.~Wilson}
\author[33]{R.~J.~Wilson}
\author[83]{L.~Winslow}
\author[35]{P.~Wittich}
\author[19]{H.~H.~Wong}
\author[119]{K.~Wood}
\author[15]{E.~Worcester}
\author[15]{M.~Worcester}
\author[145]{S.~Wu}
\author[62]{T.~Xin}
\author[125]{C.~Yanagisawa}
\author[29]{S.~Yang}
\author[43]{T.~Yang}
\author[78]{K.~Yarritu}
\author[124]{J.~Ye}
\author[15]{M.~Yeh}
\author[56]{N.~Yershov}
\author[43]{K.~Yonehara}
\author[15]{B.~Yu}
\author[129]{J.~Yu}
\author[3]{J.~Zalesak}
\author[70]{A.~Zalewska}
\author[126]{B.~Zamorano}
\author[117]{L.~Zang}
\author[107]{A.~Zani}
\author[16]{A.~Zani}
\author[46]{G.~Zavala}
\author[43]{G.~Zeller}
\author[15]{C.~Zhang}
\author[120]{C.~Zhang}
\author[32]{E.~D.~Zimmerman}
\author[116]{M.~Zito}
\author[43]{R.~Zwaska}



\affil[1]{ABC Federal University, Santo Andr\'e \textendash SP, 09210-580, Brazil}

\affil[2]{APC-Paris, Batiment Condorcet;
10, rue Alice Domon et L'eonie Duquet;
F-75205 Paris CEDEX 13, France}

\affil[3]{Institute of Physics ASCR, v. v. i. , Na Slovance 2; 182 21 Praha 8, Czech Republic}

\affil[4]{Univ. of Alabama (Tuscaloosa), Tuscaloosa, AL 35487-0324, USA}

\affil[5]{Univ. Federal de Alfenas em Po\c cos de Caldas, 11999, CEP 37715-900 Po\c cos de Caldas-MG, Brazil}

\affil[6]{Aligarh Muslim University, Department of Physics
Aligarh-202002, India}

\affil[7]{Antananarivo, , Madagascar}

\affil[8]{Argonne National Lab., Argonne, IL 60439, USA}

\affil[9]{University of Athens, University Campus, Zografou  GR 157 84
Greece, Greece}

\affil[10]{Universidad del Atlantico, Km 7 antigua vi  a Puerto Colombia, Barranquilla, Colombia}

\affil[11]{Banaras Hindu University, Dept. of Physics, Varanasi UP 221005, India}

\affil[12]{Bhabha Atmoic Research Center, , India}

\affil[13]{Univ. of Bern, Lab for High Energy Physics;
Sidlerstrasse 5; CH-3012 Bern, Switzerland}

\affil[14]{Boston University, Boston, MA 02215, USA}

\affil[15]{Brookhaven National Lab., Upton, NY 11973-5000, USA}

\affil[16]{CERN, European Organization for Nuclear Research
European Laboratory for Particle Physics; 1211 Gen`eve 23, Switzerland}

\affil[17]{CIEMAT, Divisi\'on de F\'{i}sica de Part\'{i}culas; Avenida Complutense 40; E-28040 Madrid, Spain}

\affil[18]{CNI Pisa, , Italy}

\affil[19]{University of California at Berkeley, \#7300;
Berkeley, CA 94720-7300, USA}

\affil[20]{Univ. of California (Davis), Davis, CA 95616, USA}

\affil[21]{Univ. of California (Irvine), Irvine, CA 92697-4575, USA}

\affil[22]{Univ. of California (Los Angeles), Los Angeles, CA 90095-1547, USA}

\affil[23]{California Inst. of Tech., MC 356-48;
Pasadena, CA 91125, USA}

\affil[24]{Univ. of Cambridge, JJ Thomson Avenue, Cambridge CB3 0HE, UK}

\affil[25]{Univ. de Campinas, Av. S\'ergio Buarque de Holanda, 777 CEP 13083-859 Campinas-SP, Brazil}

\affil[26]{Univ. di Catania, Via Santa Sofia, I-95123 Catania, Italy}

\affil[27]{Institute of Particle and Nuclear Physics of the Faculty of Mathematics and Physics of the Charles University in Prague, V Hole\v sovi\v ck\'ach 747/2; 180 00 Praha 8-Libe\v n, Czech Republic}

\affil[28]{Univ. of Chicago, Chicago, IL 60637-1434, USA}

\affil[29]{Univ. of Cincinnati, Cincinnati, OH 45221-0011, USA}

\affil[30]{Cinvestav, , Mexico}

\affil[31]{Universidad de Colima, Facultad de Ciencias
Bernal Diaz del Castillo 340
Colonia Villa San Sebastian
Colima, Colima, Mexico}

\affil[32]{Univ. of Colorado, Boulder, CO 80309, USA}

\affil[33]{Colorado State University, Fort Collins, CO 80523, USA}

\affil[34]{Columbia University, New York, NY 10027, USA}

\affil[35]{Cornell Univ., Laboratory for Elementary-Particle Physics; Newman Lab;
Ithaca, NY 14853\textendash5001, USA}

\affil[36]{Czech Technical University in Prague, Brehova 7; 115 19 Praha 1, Czech Republic}

\affil[37]{Dakota State University, Madison, SD 57042, USA}

\affil[38]{Univ. of Delhi, Department of Physics and Astrophysics, Delhi 110007, India}

\affil[39]{Drexel University, Philadelphia, PA 19104, USA}

\affil[40]{Duke University, Durham, NC 27706, USA}

\affil[41]{Univ. of Durham, Institute for Particle Physics Phenomenology;
Dept. of Physics, Ogden Centre for Fund. Physics;
South Road; Durham DH1 3LE, UK}

\affil[42]{Univ. Estadual de Feira de Santana, S/N;44036-900, Feira de Santana-BA, Brazil}

\affil[43]{Fermi National Accelerator Lab, Batavia, IL 60510-0500, USA}

\affil[44]{Univ. Federal de Goias, Goiania, GO, Brazil}

\affil[45]{Gran Sasso Science Institute, , Italy}

\affil[46]{Universidad de Guanajuato, Gto., C.P.37000, Mexico}

\affil[47]{Harish-Chandra Research Institute, Jhunsi, Allahabad 211 019, India}

\affil[48]{Univ. of Hawaii, Honolulu, HI 96822-2219, USA}

\affil[49]{Univ. of Houston, Houston, TX 77204, USA}

\affil[50]{Huddersfield, , UK}

\affil[51]{Horia Hulubei National Institute of Physiscs and Nuclear Engineering, Horia Hulubei National Institute of Physiscs and Nuclear
Engineering, Bucharest-Magurele, Romania}

\affil[52]{University of  Hyderabad, Gachibowli, Hyderabad - 500 046, India}
%
\affil[53]{Institut de %F\`\isica 
Fisica d'Altes Energies (IFAE); Campus Universitat Autonoma de Barcelona , E-08193  Cerdanyola del Valles (Barcelona), Spain}

\affil[54]{Illinois Institute of Technology , Room 182LS; Chicago, IL 60616, USA}

\affil[55]{IIT Hyderabad, Kandi, Hyderabad - 502205, India}

\affil[56]{Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), 60th October Anniversary Prosp. 7a
Moscow, Russia 117312, Russia}

\affil[57]{Institute for Research in Fundamental Sciences (IPM), Tehran, Iran.
Postal code: 19538-33511
PO Box: 19395-5531, Iran}

\affil[58]{Idaho State University, Department of Physics
921 South 8th Ave.
Stop 8106
Pocatello, ID 83209-8106, USA}

\affil[59]{Imperial College of Science Tech. \& Medicine, Blackett Lab.; Prince Consort Road; London SW7 2BZ, UK}

\affil[60]{Indian Institute of Technology Guwahati, Guwahati, 781 039, India}

\affil[61]{Indiana University, Bloomington, IN 47405-7105, USA}

\affil[62]{Iowa State University, Ames, IA 50011, USA}

\affil[63]{Institut de Physique Nucleaire de Lyon (IPNL), Rue E. Fermi 4
69622 Villeurbanne, France}

\affil[64]{University of Jammu, Physics Department, JAMMU-180006, India}

\affil[65]{Kansas State University, Manhattan, KS 66506, USA}

\affil[66]{Kavli IPMU, Univ. of Tokyo, Kashiwa Shi, Chiba 277-8568, Japan}

\affil[67]{KEK, High Energy Accelerator Research Organization
1\textendash1 Oho, Tsukuba-shi; Ibaraki-ken 305-0801, Japan}

\affil[68]{KYIV National University, Department of Nuclear Physics, 64, 01601 Kyiv, Ukraine}

\affil[69]{Koneru Lakshmaiah, , India}

\affil[70]{Krakow, , Poland}

\affil[71]{Lab. d'Annecy-le-Vieux de Phys. des Particules, BP 110; F-74941 Annecy-le-Vieux CEDEX, France}

\affil[72]{Laboratori Nazionali del Gran Sasso, I-67010 Assergi, AQ, Italy}

\affil[73]{Lancaster University, Bailrigg, Lancaster LA1 4YB, UK}

\affil[74]{Lawrence Berkeley National Lab., Berkeley, CA 94720-8153, USA}

\affil[75]{Universit\'e de Li\`ege, Bat B5, Sart Tilman B-4000, Belgium}

\affil[76]{Univ. of Liverpool, L69 7ZE, Liverpool, UK}

\affil[77]{University College London, London, WC1E 6BT, UK}

\affil[78]{Los Alamos National Laboratory, Los Alamos, NM 87545, USA}

\affil[79]{Louisiana State University, Baton Rouge, LA 70803-4001, USA}

\affil[80]{University of Lucknow, Department of Physics
Lucknow 226007
Uttar Pradesh, India}

\affil[81]{Univ. of Manchester, Oxford Road, Manchester M13 9PL, UK}

\affil[82]{Univ. of Maryland, College Park, MD 20742-4111, USA}

\affil[83]{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}

\affil[84]{Univ. of Puerto Rico, Box 9016; Mayaguez, PR 00681-9000, USA}

\affil[85]{University of Michigan, 450 Church Street
Ann Arbor, Michigan 48109-1040, USA}

\affil[86]{Michigan State University, East Lansing, MI 48824, USA}

\affil[87]{Univ. di Milano, INFN Sezione di Milano, I-20133 Milano, Italy}

\affil[88]{INFN Sezione di Milano Bicocca, Piazza della Scienza 3, 20126 Milano, Italy}

\affil[89]{Univ. of Minnesota, Minneapolis, MN 55455, USA}

\affil[90]{Univ. of Minnesota (Duluth), Duluth, MN 55812, USA}

\affil[91]{NIKHEF, Science Park, Amsterdam, Netherlands}

\affil[92]{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy}

\affil[93]{National Centre for Nuclear Research, A. Soltana 7, 05 400 Otwock, Poland}

\affil[94]{Jawaharlal Nehru University, New Delhi 110067, INDIA, India}

\affil[95]{Univ. of New Mexico, MSC07 4220;
Albuquerque, NM 87131, USA}

\affil[96]{Northwestern University, Evanston, Il 60208, USA}

\affil[97]{Univ. of Notre Dame, Notre Dame, IN 46556-5670, USA}

\affil[98]{Observatorio Nacional, , Brazil}

\affil[99]{Ohio State Univ., Dept. of Physics; 191 W. Woodruff Ave.;
Columbus, OH 43210, USA}

\affil[100]{Oregon State University, Dept. of Physics;
301 Weniger Hall; Corvallis, OR 97331\textendash6507, USA}

\affil[101]{Univ. of Oxford, Oxford, OX1 3RH, UK}

\affil[102]{Pacific Northwest National Lab, , USA}

\affil[103]{Pennsylvania State University, PMB 264;
University Park, PA 16802-6300, USA}

\affil[104]{PUCP, , Peru}

\affil[105]{Univ. of Padova, Dip. Fisica e Astronomia G. Galilei and INFN Sezione di
Padova, I-35131 Padova, Italy}

\affil[106]{Panjab University, Chandigarh, 160014 U.T., India}

\affil[107]{Univ. of Pavia, INFN Sezione di Pavia, I-27100 Pavia, Italy}

\affil[108]{Univ. of Pennsylvania, Philadelphia, PA 19104-6396, USA}

\affil[109]{Univ. di Pisa, Theor. Division;
Largo B. Pontecorvo 3, Ed. B-C; I-56127 Pisa, Italy}

\affil[110]{Univ. of Pittsburgh, Pittsburgh, PA 15260, USA}

\affil[111]{Princeton University, Princeton, New Jersey 08544-0708, USA}

\affil[112]{Punjab Agri. University, Centre for High Energy Physics;
Lahore - 54590, India}

\affil[113]{Univ. of Rochester, Rochester, NY 14627-0171, USA}

\affil[114]{SLAC National Acceleratory Laboratory, Menlo Park, CA 94025, USA}

\affil[115]{STFC Rutherford Appleton Laboratory, Harwell Oxford, Didcot OX11 0QX, UK}

\affil[116]{CEA/Saclay, IPhT; Inst. de Physique Theorique;
Orme des Merisiers, Point Courrier 136;
F-91191 Gif-sur-Yvette CEDE, France}

\affil[117]{Univ. of Sheffield, Sheffield, S3 7RH, UK}

\affil[118]{Univ. of Sofia, Atomic Physics Dept., Faculty of Physics;
5 James Bourchier Blvd.; BG-1164 Sofia, Bulgaria}

\affil[119]{Univ. of South Carolina, Columbia, SC 29208, USA}

\affil[120]{Univ. of South Dakota, Vermillion, SD 57069, USA}

\affil[121]{South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}

\affil[122]{South Dakota Science And Technology Authority, Lead, SD 57754, USA}

\affil[123]{South Dakota State University, Brookings, SD 57007, USA}

\affil[124]{Southern Methodist University, Dallas, TX 75275, USA}

\affil[125]{Stony Brook University, Nucleon Decay and Neutrino Physics Group
Department of Physics and Astronomy
Stony Brook University
Stony Brook, NY 11794-3800, USA}

\affil[126]{Univ. of Sussex, Brighton, BN1 9RH, UK}

\affil[127]{Syracuse University, Syracuse, NY 13244-1130, USA}

\affil[128]{Univ. of Tennessee at Knoxville, Knoxville, TN, USA}

\affil[129]{Univ. of Texas (Arlington), Arlington, TX 76019, USA}

\affil[130]{Univ. of Texas (Austin), Austin, TX 78712-0264, USA}

\affil[131]{TUBITAK Space Technologies Research Institute , TR-06800, Ankara, Turkey}

\affil[132]{Tufts University, Medford, MA 02155, USA}

\affil[133]{Variable Energy Cyclotron Centr, , India}

\affil[134]{Instituto de Fisica Corpuscular, C/Catedratico Jose Beltran, 2
E-46980 Paterna (Valencia), Spain}

\affil[135]{Virginia Tech., Blacksburg, VA 24061-0435, USA}

\affil[136]{Univ. of Warsaw, Faculty of Physics 
ul. Pasteura 5
02-093 Warsaw, Poland}

\affil[137]{Univ. of Warwick, Coventry CV4 7AL, UK}

\affil[138]{Wichita State University, Physics Division
1845 Fairmount St.
Wichita, KS 67260-0032, USA}

\affil[139]{College of William and Mary, Williamsburg, VA 23187-8795, USA}

\affil[140]{Univ. of Wisconsin, Madison, WI 53706, USA}

\affil[141]{Wroclaw University, Plac Maxa Borna 9, 50-204 Wroclaw, Poland}

\affil[142]{Yale University, New Haven, CT 06520, USA}

\affil[143]{Yerevan Institute for Theoretical Physics and Modeling, Halabian Str. 34; Yerevan 0036, Armenia}

\affil[144]{York, Physics and Astronomy Dept.;
4700 Keele St.; Toronto M3J 1P3, Canada}

\affil[145]{ETH Zurich, HPK F 23
Schafmattstr. 20
8093 Z\"urich, Switzerland}



